Fine-Pruning: Defending Against Backdooring Attacks on Deep Neural Networks

Deep neural networks (DNNs) provide excellent performance across a wide range of classification tasks, but their training requires high computational resources and is often outsourced to third parties. Recent work has shown that outsourced training introduces the risk that a malicious trainer will return a backdoored DNN that behaves normally on most inputs but causes targeted misclassifications or degrades the accuracy of the network when a trigger known only to the attacker is present. In this paper, we provide the first effective defenses against backdoor attacks on DNNs. We implement three backdoor attacks from prior work and use them to investigate two promising defenses, pruning and fine-tuning. We show that neither, by itself, is sufficient to defend against sophisticated attackers. We then evaluate fine-pruning, a combination of pruning and fine-tuning, and show that it successfully weakens or even eliminates the backdoors, i.e., in some cases reducing the attack success rate to 0% with only a 0.4% drop in accuracy for clean (non-triggering) inputs. Our work provides the first step toward defenses against backdoor attacks in deep neural networks.

==> outline.tex <==
--- Introduction (BDG)
      What are Backdoor attacks?
      Based on characteristics of backdoor attacks, pruning natural defense
      We show: 1. pruning works on the baseline attack; 2. advance attacker can evade pruning; 3. fine-tuning defense works.
      
--- Background (SG)
     2.1 What are NNs (SG)
     2.2 Backdoor Attacks (SG)
         2.2.1 Attack Model (SG)
     2.3 Examples of Backdoor Attacks (KL)
            --- Traffic Sign
            --- Face
            --- Speech

--- Methodology (KL/SG/BDG)
       --- Pruning Defense 
           -- How does pruning defense work?
           -- Experimental Results
           
       --- Adaptive Attacker
           -- how does an adaptive attacker respond to pruning defense
           -- Experiemntal results
           
       --- Fine-tuning defense 
          -- how does fine-tuning work
          -- Experimental results

--- Discussion (SG)
 
--- Related Work (BDG)
